Controlling swarms towards flocks and mills

Self-organization and control around flocks and mills is studied for second-order swarming systems involving self-propulsion and potential terms. It is shown that through the action of constrained control, is it possible to control any initial configuration to a flock or a mill. The proof builds on an appropriate combination of several arguments: LaSalle invariance principle and Lyapunov-like decreasing functionals, control linearization techniques, and quasi-static deformations. A stability analysis of the second-order system guides the design of feedback laws for the stabilization to flock and mills, which are also assessed computationally.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi


%%%%ours

\usepackage{amsmath,amssymb}
%\usepackage{subfigure,float,url,color}
\usepackage{lmodern,tikz}
%\usetikzlibrary{patterns}
\usepackage{enumitem}
%\usepackage{mathrsfs}
%\usepackage[colorlinks=true]{hyperref}
%\usepackage{pdfsync}
%\usepackage{showkeys}
%\usepackage{refcheck}

\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}

\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}

%\newtheorem{theorem}{Theorem}  
%\newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
%\theoremstyle{definition}
%\newtheorem{remark}{Remark}


\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\weak}{\rightharpoonup}
\newcommand{\dt}{\tau}
\newcommand{\al}{\alpha}
\newcommand{\X}{\mathcal{X}}
\newcommand{\FR}[1]{{\textcolor{red}{#1}}}
\newcommand{\FRc}[1]{\footnote{\textcolor{red}{#1}}}
\newcommand{\Pt}[1]{\left({#1}\right)}
\newcommand{\eps}{\varepsilon}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\grad}{\nabla}
\newcommand{\nn}{\nonumber\\}
\newcommand{\albe}{\sqrt\frac{4\alpha^{3}}{27\beta} }

\graphicspath{{Figs/}}



%\topmargin -1cm
%\textheight 21cm
%\textwidth 15cm 
%\oddsidemargin 1cm




% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}




% Sets running headers as well as PDF title and authors
\headers{Controlling swarms towards flocks and mills}{J.A. Carrillo, D. Kalise, F. Rossi and E. Tr\'elat}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Controlling swarming models \\ towards flocks and mills\thanks{Submitted to the editors DATE.
\funding{JAC was supported the Advanced Grant Nonlocal-CPD (Nonlocal PDEs for Complex Particle Dynamics: Phase Transitions, Patterns and Synchronization) of the European Research Council Executive Agency (ERC) under the European Union's Horizon 2020 research and innovation programme (grant agreement No. 883363). JAC was also partially supported by the EPSRC grant number EP/P031587/1 and EP/T022132/1. \\
DK was supported by a public grant as part of the Investissement d’avenir project,reference ANR-11-LABX-0056-LMH, LabEx LMH, and by the UK Engineering and Physical Sciences Research Council (EPSRC) grants EP/V04771X/1, EP/T024429/1, and EP/V025899/1. \\
FR was supported by the University of Padua under the STARS Grants programme CONNECT: Control of Nonlocal Equations for Crowds and Traffic models. \\
ET was supported by the grant ANR-20-CE40-0009-04 TRECOS (New Trends in Control and Stabilization: Constraints and Non-local terms).
}
}}

% Authors: full names plus addresses.
\author{Jos\'e A. Carrillo\thanks{Mathematical Institute, University of Oxford, Oxford OX2 6GG, UK (\texttt{carrillo@maths.ox.ac.uk}).}
	\and
	Dante Kalise\thanks{School of Mathematical Sciences, University of Nottingham, UK (\texttt{dante.kalise@nottingham.ac.uk}).}
	\and
	Francesco Rossi\thanks{Dipartimento di Matematica ``Tullio Levi-Civita'', Universit\`a\ degli Studi di Padova, Via Trieste 63, 35121 Padova, Italy  (\texttt{francesco.rossi@math.unipd.it}).}
	\and
	Emmanuel Tr\'elat\thanks{Sorbonne Universit\'e, CNRS, Universit\'e de Paris, Inria, Laboratoire Jacques-Louis Lions (LJLL), F-75005 Paris, France (\texttt{emmanuel.trelat@sorbonne-universite.fr}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

